Optimistic Verifiable Training by Controlling Hardware Nondeterminism

The increasing compute demands of AI systems have led to the emergence of services that train models on behalf of clients lacking necessary resources. However, ensuring correctness of training and guarding against potential training-time attacks, such as data poisoning and backdoors, poses challenges. Existing works on verifiable training largely fall into two classes: proof-based systems, which are difficult to scale, and ``optimistic'' methods that consider a third-party auditor who can replicate the training process and contest the trainer. A key challenge with the latter is that nondeterminism between GPU types during training prevents exact replication of the training process, resulting in schemes that are non-robust. We propose a method that combines training in a higher precision than the target, rounding after intermediate computations, and sharing rounding decisions based on an adaptive thresholding procedure, to successfully control for nondeterminism. Across three different NVIDIA GPUs (A40, Titan XP, RTX 2080 Ti), we achieve exact training replication at FP32 precision for both full-training and fine-tuning of ResNet-50 (23M) and GPT-2 (117M) models. Our verifiable training scheme significantly decreases the storage and time costs compared to proof-based systems, and is publicly released at https://github.com/meghabyte/verifiable-training.

==> scratch/alternates.tex <==
\begin{itemize}
    \item One approach is to train on one hardware (e.g. A100) and verify on another (e.g. V100).
    \item Another approach is to train on a large amount of one hardware (e.g. 1000 A100s) and verify on a small amount of that hardware (e.g. 8 A100s). \megha{does this create any research question issues, or just an example situation? i guess maybe the parellilism can be a cause of non-determinism?}
    \item Can the prover do side-computations (e.g. certify matmul somehow) to reduce the verifier load? 
    \item Is it possible to simulate a V100's mode of operation using an A100? Does our setting permit the verifier to run much more slowly? \megha{yes i think its ok for the verifier to take the time they need}
    % https://people.ece.ubc.ca/aamodt/papers/accelsim.isca2020.pdf (GPGPUsim -- a system for simulating GPUs)
    \item Could the verifier repeat computation e.g., repeat a layer 3$\times$ and average over them or check if any of them match the prover's result?
    \item Could you verify that a model wasn't trained on some website or something?
\end{itemize}

==> scratch/background.tex <==

\subsection{Hardware Landscape} 
There are many kinds of GPUs what are the differences? What is the difference between Tesla and RTX? RTX is one visual computing platform that runs on Volta-, Turing-, Ampere- micro-architectures using the Tensor Cores.


\subsection{Hardware Execution}

In GPUs, thread is a stream of instructions and data that is assigned to one CUDA core --- a single instruction applies to multple threads (SIMT) and acts on multiple data. CUDA core processes the data item to exeute its portion of a SIMT instruction stream. CUDA cores work in teams of 32, executing the same instruction stream, on different data (a warp is a group of 32 threads), called SIMD (Single Instruction on Multiple Data) parallelism. A kernel is a function that runs on the device and it can be broken up into thread blocks. A streaming multiprocessor (SM) is a unit that can execute a thread block (piece) of a kernel. See \cite{lantz2021understanding} for more information. 

\input{tables/devices}
\paragraph{Matrix multiplications} Recall matmul comprises multiplication and addition operations --- each small product results in a value that has to be stored somewhere, before it can be accumulated with other products (requires lots of registers, reads, and writes). GPUs support GEMM (Genral Matrix Multiplication): a fused operation for $\mathbf{D} = (\mathbf{A} \times \mathbf{B}) + \mathbf{C}$, note the operation is 3 FLOPs; $\mathbf{A}$ and $\mathbf{B}$ are input matrices with shapes $m \times k$ and $k \times n$, $\mathbf{C}$ is the accumulator.  Tensor cores are dedicated matmul units to provide massive computation throughput. Tensor cores are designed to execute $K$ GEMMs per clock cycle on $N \times N$ matrices containing values in some data format (e.g. INT8, FP16) --- since actual matrices can be larger than $N$ dimension, the matrices are split into blocks and then built up to the final answer. Note that in contrast to Tensor cores, which perform multiple operatoins per clock cycle, GPUs also have more general purpose CUDA cores, which perform one operation per clock cycle.

Note all GPUs do not have Tensor cores (Pascal architectures), some do (Turing architectures). Different GPUs can have different numbers of cores, which affects the level of parallelism that is supported. TPUs a use deterministic, single-threaded computation model in contrast to CPUs and GPUs --- this is enabled since they use systolic arrays in matrix unit. \yell{Does this make TPUs a good candidate for us? What are systolic arrays?}

\yell{Does the for non-determinism relies on the fact that Tensor cores fall back on non-deterministic CUDA cores for computations they do not themselves support?} 

\paragraph{Streaming Multiprocessor (SM)} Fundamental GPU processing units. They are connected to the GPU device / global memory, but also have their own internal caches, shared memory, register file, CUDA cores, Tensor cores, load store units, other special units. The two types of instruction execution schemes that the SM can use are \textit{per-thread}, i.e. instruction is executed by a single thread independently and the behavior/result of the thread is deterministic, and \textit{per-warp}, i.e.  instruction is executed by the 32 threads within the same warp cooperatively and the behavior/results are not deterministic.

\paragraph{HMMA.884 SASS} HMMA.884 seems to be the fundamental instruction set that the GPU compiles to. TCs on different GPU architectures compile differently \cite{sun2022dissecting}.

\paragraph{Data Movement} We need to move data back and forth between the host and GPU. Do we need to worry about the data ordering at all? 

\subsection{Sources of Non-Determinism} Implementation and hardware architecture sources of non-determinism. At a high level different floating point accumulation orders can change the result. \yell{Things to read up on: Kahan summation.} 
For distributed training we introduce networks communication. We would need to enforce a particular ordering of packets. 

Algorithm sources of non-determinism: data ordering and augmentations, parameter initialization and regularization.

\subsection{Measures of Model Stability}
\megha{I think for our application we need the weights to be exact, unless we consider as an additional think some kind of likelihood proof under a bounded notion of a stability}

\paragraph{Churn} Defined as the fraction of test examples where the predictions of two models $f_1$ and $f_2$ disagree. 

\paragraph{L2 norm} L2 norm of the trained weights $||w_1^* - w_2^*||$ between $f_1$ and $f_2$ at the end of training indicates the divergence of each run in the function space. 

\paragraph{Standard Deviation} Standard deviation in top-1 test-set performance over independent runs. Can also look at sub-group performance.

\subsection{Memory Requirements}
What can we actually store in a Merkle tree? For a 1B parameter model, trained over 300B tokens, we couldn't store information for every step could we? Where can we checkpoint? One approach to address this is also to hash multiple times. 

==> scratch/notes.tex <==

\section{Alternate Set-Ups for the Prover and Verifier}
\input{scratch/alternates}

\section{Background}
\input{scratch/background}




==> tables/devices.tex <==
\begin{table}[t]
\centering
% \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
\begin{tabular}{lccc}
\hline
Device  & Architecture & TCs/SM & TC MM $m \times n \times k$ \\
\hline
A100 &  Ampere  & 4 & 8 $\times$ 4 $\times$ 8\\
V100 &  Volta  & 8 & 4 $\times$ 4 $\times$ 4\\
Titan-XP  & Pascal & -  & \\
A40       & Ampere &  & \\
\hline
\end{tabular}
\caption{Relevant properties of the GPU architectures we're using. TC stands for Tensor Core.}
\label{tab:device-properties}
\end{table}

==> tables/floating_point_examples.tex <==
\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{ccccc}
\toprule
\textbf{Example}  & 
\textbf{Summation Order} & 
\textbf{FP32} &
\textbf{FP32 Rounded to FP16} \\ 
\midrule
\multirow{2}{*}{
$a,b,c=0.1, -0.1, 0.2$
} 
& $a+b+c$  
& 00111110010011001100110011001101   
& 0011001001100110 \\
& $a+c+b$  
& 00111110010011001100110011001110   
& 0011001001100110 \\

\midrule
\multirow{2}{*}{
$a,b,c=10.02,13.162813186645508,0.2$
} 
& $a+b+c$  
& 01000001101110110001000000000001  
& 0100110111011001  \\
& $a+c+b$  
& 01000001101110110001000000000000   
& 0100110111011000 \\

\bottomrule                                           
\end{tabular}
\caption{Two examples of floating point accumulation error when rounding arithmetic performed higher precision (e.g. FP32) down to lower precision (e.g. FP16). In the first example, error in the FP32 result \textit{does not} transfer to the rounded FP16 result. In the second example, the errror in the FP32 result \textit{does} transfer to the rounded result.}
\label{tab:floating_point_a}
\end{table*}


